Improving Slot Filling Performance with Attentive Neural Networks on Dependency Structures

Slot Filling (SF) aims to extract the values of certain types of attributes (or slots, such as person:cities\_of\_residence) for a given entity from a large collection of source documents. In this paper we propose an effective DNN architecture for SF with the following new strategies: (1). Take a regularized dependency graph instead of a raw sentence as input to DNN, to compress the wide contexts between query and candidate filler; (2). Incorporate two attention mechanisms: local attention learned from query and candidate filler, and global attention learned from external knowledge bases, to guide the model to better select indicative contexts to determine slot type. Experiments show that this framework outperforms state-of-the-art on both relation extraction (16\% absolute F-score gain) and slot filling validation for each individual system (up to 8.5\% absolute F-score gain).

==> 2hypotheses.tex <==
\section{Motivations}

We then use some real examples to explain and motivate our approach.

Dependency parsing based features, especially the shortest dependency path between two entities, have been proved to be effective to extract the most important information for identifying the relation between two entities~\cite{bunescu2005shortest,zhao2005extracting,guodong2005exploring,jiang2007systematic}. Several recent studies also explored transforming a  dependency path into a sequence and applied Neural Networks to the sequence for relation classification~\cite{Liu2015,caibidirectional,xu2015classifying}. 

However, for SF, the shortest dependency path between query and candidate filler is not always sufficient to infer the slot type due to two reasons. \heng{add some statistics to show how many instances cannot be captured by this simplistic previous approach} First, the most indicative words may not be included in the path. For example, in the following sentence: 

\begin{enumerate}[label={E}\arabic*.]\setcounter{enumi}{1}
\item Survivors include two \textit{sons} and \textit{daughters}-in-law, \textbf{Troy}$_{filler}$ and Phyllis Perry, \textbf{Kenny}$_{query}$ and Donna Perry, all of Bluff City.
\end{enumerate}

the shortest dependency path between \textbf{Kenny} and \textbf{Troy} is:
``Troy $\leftarrow^{conj}$ Perry $\leftarrow^{conj}$ Kenny'', which does not include the most indicative words: \textit{sons} and \textit{daughters} for their \textit{per:siblings} relation. 
In addition, the relation between query and candidate filler is also highly related to their entity types, especially for disambiguating slot types such as \textit{per:country\_of\_birth} \textit{per:state\_of\_birth} and \textit{per:city\_of\_birth}. Entity types can be inferred by enriching query and filler related contexts. For example, in the following sentence: 

\begin{enumerate}[label={E}\arabic*.]\setcounter{enumi}{2}
\item \textbf{Merkel}$_{query}$ was died in the southern German city of \textbf{Passau}$_{filler}$ in 1967.
\end{enumerate}

we can determine the slot type as  \textit{city} related by incorporating rich contexts (e.g., ``\textit{city}''). 



